A joint test of unconfoundedness and common trends

This paper introduces an overidentification test of two alternative assumptions to identify the average treatment effect on the treated in a two-period panel data setting: unconfoundedness and common trends. Under the unconfoundedness assumption, treatment assignment and post-treatment outcomes are independent, conditional on control variables and pre-treatment outcomes, which motivates including pre-treatment outcomes in the set of controls. Conversely, under the common trends assumption, the trend and the treatment assignment are independent, conditional on control variables. This motivates employing a Difference-in-Differences (DiD) approach by comparing the differences between pre- and post-treatment outcomes of the treatment and control group. Given the non-nested nature of these assumptions and their often ambiguous plausibility in empirical settings, we propose a joint test using a doubly robust statistic that can be combined with machine learning to control for observed confounders in a data-driven manner. We discuss various causal models that imply the satisfaction of either common trends, unconfoundedness, or both assumptions jointly, and we investigate the finite sample properties of our test through a simulation study. Additionally, we apply the proposed method to five empirical examples using publicly available datasets and find the test to reject the null hypothesis in two cases.

==> Output/Tables/01_LaLonde/lalondetable_nswpsid.tex <==
% latex table generated in R 4.2.2 by xtable 1.8-4 package
% Tue Jun 11 11:24:35 2024
\begin{tabularx}{\textwidth}{l*{7}{Y}}
   \toprule
  \toprule 
 & \multicolumn{3}{c}{\textit{Test results}} & \multicolumn{2}{c}{$Unconf$} & \multicolumn{2}{c}{$DiD$} \\
 \cmidrule(lr){2-4} \cmidrule(lr){5-6} \cmidrule(lr){7-8} 
Learner & $\hat{\theta}$ & SE & p-val & $\hat{\Delta}_{Unconf}$ & SE & $\hat{\Delta}_{DiD}$ & SE \\
 \cmidrule(lr){1-4} \cmidrule(lr){5-6} \cmidrule(lr){7-8}   Ensemble & 1568.314 & 404.668 & 0.000 & -1417.299 & 780.464 &  151.015 &  715.693 \\ 
  Lasso & 1944.306 & 681.185 & 0.004 &  -556.234 & 816.370 & 1388.072 & 1102.786 \\ 
  Parametric & 2233.996 & 840.595 & 0.008 &  -522.710 & 841.478 & 1711.286 & 1235.235 \\ 
  RF & 2314.383 & 524.875 & 0.000 & -2109.356 & 759.806 &  205.028 &  682.622 \\ 
   \bottomrule
\end{tabularx}



==> Output/Tables/02_JC/misc/JChealthtable.tex <==
% latex table generated in R 4.3.1 by xtable 1.8-4 package
% Thu May 23 18:32:07 2024
\begin{tabularx}{\textwidth}{l*{7}{Y}}
   \toprule
  \toprule 
 & \multicolumn{3}{c}{\textit{Test results}} & \multicolumn{2}{c}{$Unconf$} & \multicolumn{2}{c}{$DiD$} \\
 \cmidrule(lr){2-4} \cmidrule(lr){5-6} \cmidrule(lr){7-8} 
Learner & $\hat{\theta}$ & SE & p-val & $ATET_{Unconf}$ & SE & $ATET_{DiD}$ & SE \\
 \cmidrule(lr){1-4} \cmidrule(lr){5-6} \cmidrule(lr){7-8}   Ensemble & -0.062 & 0.017 & 0.000 & -0.030 & 0.018 & -0.092 & 0.024 \\ 
  Lasso & -0.047 & 0.016 & 0.004 & -0.036 & 0.017 & -0.083 & 0.023 \\ 
  Parametric & -0.049 & 0.017 & 0.003 & -0.036 & 0.017 & -0.085 & 0.023 \\ 
  RF & -0.083 & 0.030 & 0.006 & -0.022 & 0.025 & -0.105 & 0.038 \\ 
  SVM & -0.062 & 0.017 & 0.000 & -0.020 & 0.016 & -0.082 & 0.022 \\ 
  XGBoost & -0.066 & 0.029 & 0.023 & -0.012 & 0.025 & -0.078 & 0.037 \\ 
   \bottomrule
\end{tabularx}



==> Output/Tables/02_JC/misc/JCpworkytable.tex <==
% latex table generated in R 4.3.1 by xtable 1.8-4 package
% Thu May 23 17:47:44 2024
\begin{tabularx}{\textwidth}{l*{7}{Y}}
   \toprule
  \toprule 
 & \multicolumn{3}{c}{\textit{Test results}} & \multicolumn{2}{c}{$Unconf$} & \multicolumn{2}{c}{$DiD$} \\
 \cmidrule(lr){2-4} \cmidrule(lr){5-6} \cmidrule(lr){7-8} 
Learner & $\hat{\theta}$ & SE & p-val & $ATET_{Unconf}$ & SE & $ATET_{DiD}$ & SE \\
 \cmidrule(lr){1-4} \cmidrule(lr){5-6} \cmidrule(lr){7-8}   Ensemble & 3.462 & 0.435 & 0.000 & 4.037 & 0.828 & 7.499 & 0.884 \\ 
  Lasso & 3.533 & 0.396 & 0.000 & 3.908 & 0.813 & 7.440 & 0.869 \\ 
  Parametric & 3.463 & 0.392 & 0.000 & 3.958 & 0.818 & 7.421 & 0.874 \\ 
  RF & 3.203 & 0.785 & 0.000 & 4.819 & 1.105 & 8.022 & 1.174 \\ 
  SVM & 4.166 & 0.405 & 0.000 & 3.810 & 0.789 & 7.975 & 0.826 \\ 
  XGBoost & 2.646 & 1.143 & 0.021 & 4.209 & 1.298 & 6.855 & 1.282 \\ 
   \bottomrule
\end{tabularx}



==> Output/Tables/04_njmin/njmin_EMPPT.tex <==
% latex table generated in R 4.3.1 by xtable 1.8-4 package
% Mon May 27 12:14:44 2024
\begin{tabularx}{\textwidth}{l*{7}{Y}}
   \toprule
  \toprule 
 & \multicolumn{3}{c}{\textit{Test results}} & \multicolumn{2}{c}{$Unconf$} & \multicolumn{2}{c}{$DiD$} \\
 \cmidrule(lr){2-4} \cmidrule(lr){5-6} \cmidrule(lr){7-8} 
Learner & $\hat{\theta}$ & SE & p-val & $\hat{\Delta}_{Unconf}$ & SE & $\hat{\Delta}_{DiD}$ & SE \\
 \cmidrule(lr){1-4} \cmidrule(lr){5-6} \cmidrule(lr){7-8}   Ensemble & -0.197 & 0.503 & 0.695 & -0.527 & 1.523 & -0.724 & 1.850 \\ 
  Lasso & -1.714 & 1.303 & 0.188 &  0.251 & 1.100 & -1.463 & 1.911 \\ 
  Parametric &  0.000 & 0.000 & 0.880 & -1.121 & 3.268 & -1.121 & 3.268 \\ 
  RF & -2.344 & 2.067 & 0.257 &  0.014 & 1.567 & -2.330 & 3.306 \\ 
   \bottomrule
\end{tabularx}



==> Output/Tables/04_njmin/njmin_EMPTOT.tex <==
% latex table generated in R 4.3.1 by xtable 1.8-4 package
% Mon May 27 12:29:31 2024
\begin{tabularx}{\textwidth}{l*{7}{Y}}
   \toprule
  \toprule 
 & \multicolumn{3}{c}{\textit{Test results}} & \multicolumn{2}{c}{$Unconf$} & \multicolumn{2}{c}{$DiD$} \\
 \cmidrule(lr){2-4} \cmidrule(lr){5-6} \cmidrule(lr){7-8} 
Learner & $\hat{\theta}$ & SE & p-val & $\hat{\Delta}_{Unconf}$ & SE & $\hat{\Delta}_{DiD}$ & SE \\
 \cmidrule(lr){1-4} \cmidrule(lr){5-6} \cmidrule(lr){7-8}   Ensemble &  1.175 & 0.933 & 0.208 &  2.483 & 1.145 &  3.658 & 1.840 \\ 
  Lasso & -0.038 & 0.111 & 0.733 &  3.796 & 2.418 &  3.758 & 2.367 \\ 
  Parametric &  0.000 & 0.000 & 0.723 & -3.754 & 4.166 & -3.754 & 4.166 \\ 
  RF &  0.105 & 0.192 & 0.583 &  2.434 & 1.159 &  2.539 & 1.109 \\ 
   \bottomrule
\end{tabularx}



==> Output/Tables/04_njmin/njmin_NMGRS.tex <==
% latex table generated in R 4.3.1 by xtable 1.8-4 package
% Mon May 27 12:22:02 2024
\begin{tabularx}{\textwidth}{l*{7}{Y}}
   \toprule
  \toprule 
 & \multicolumn{3}{c}{\textit{Test results}} & \multicolumn{2}{c}{$Unconf$} & \multicolumn{2}{c}{$DiD$} \\
 \cmidrule(lr){2-4} \cmidrule(lr){5-6} \cmidrule(lr){7-8} 
Learner & $\hat{\theta}$ & SE & p-val & $\hat{\Delta}_{Unconf}$ & SE & $\hat{\Delta}_{DiD}$ & SE \\
 \cmidrule(lr){1-4} \cmidrule(lr){5-6} \cmidrule(lr){7-8}   Ensemble & -0.125 & 0.109 & 0.253 &  0.324 & 0.165 &  0.200 & 0.141 \\ 
  Lasso & -0.025 & 0.082 & 0.756 &  0.024 & 0.184 & -0.002 & 0.224 \\ 
  Parametric &  0.000 & 0.000 & 0.856 & -0.323 & 0.329 & -0.323 & 0.329 \\ 
  RF & -0.210 & 0.107 & 0.049 &  0.371 & 0.199 &  0.161 & 0.164 \\ 
   \bottomrule
\end{tabularx}



==> Output/Tables/4_Simulation/simtable.tex <==
% latex table generated in R 4.2.2 by xtable 1.8-4 package
% Fri Mar 22 06:08:12 2024
\begin{tabularx}{\textwidth}{*{11}{Y}}
   \toprule
  \toprule
\multicolumn{2}{c}{Sim. par.} & \multicolumn{5}{c}{Test} & \multicolumn{2}{c}{Selobs} & \multicolumn{2}{c}{DiD} \\
\cmidrule(lr){1-2} \cmidrule(lr){3-7} \cmidrule(lr){8-9} \cmidrule(lr){10-11}
$\gamma$ & $\delta$ & Mean $\hat{\theta}$ & Std. $\hat{\theta}$ & Mean SE $\hat{\theta}$ & Mean p-val & Reject & Bias & RMSE & Bias & RMSE \\ \midrule
0.00 & 0.00 & 0.02 & 0.10 & 0.08 & 0.42 & 0.11 & 0.13 & 0.19 & 0.15 & 0.22 \\ 
  0.03 & 0.03 & -0.05 & 0.10 & 0.08 & 0.41 & 0.13 & 0.16 & 0.21 & 0.11 & 0.20 \\ 
  0.05 & 0.05 & -0.12 & 0.10 & 0.09 & 0.27 & 0.32 & 0.19 & 0.23 & 0.07 & 0.18 \\ 
  0.05 & 0.00 & -0.03 & 0.10 & 0.08 & 0.44 & 0.11 & 0.18 & 0.23 & 0.15 & 0.22 \\ 
  0.07 & 0.00 & -0.05 & 0.10 & 0.08 & 0.42 & 0.13 & 0.20 & 0.24 & 0.15 & 0.22 \\ 
  0.10 & 0.00 & -0.07 & 0.10 & 0.08 & 0.37 & 0.19 & 0.23 & 0.27 & 0.15 & 0.22 \\ 
  0.20 & 0.00 & -0.16 & 0.10 & 0.09 & 0.17 & 0.48 & 0.31 & 0.34 & 0.15 & 0.22 \\ 
  0.25 & 0.00 & -0.20 & 0.10 & 0.09 & 0.10 & 0.65 & 0.35 & 0.38 & 0.15 & 0.22 \\ 
  0.00 & 0.05 & -0.07 & 0.10 & 0.08 & 0.37 & 0.18 & 0.14 & 0.20 & 0.07 & 0.18 \\ 
  0.00 & 0.07 & -0.12 & 0.10 & 0.09 & 0.28 & 0.32 & 0.14 & 0.20 & 0.03 & 0.17 \\ 
  0.00 & 0.10 & -0.16 & 0.10 & 0.09 & 0.18 & 0.47 & 0.14 & 0.20 & -0.02 & 0.16 \\ 
  0.00 & 0.20 & -0.33 & 0.10 & 0.10 & 0.02 & 0.91 & 0.15 & 0.21 & -0.18 & 0.24 \\ 
  0.00 & 0.25 & -0.41 & 0.11 & 0.10 & 0.01 & 0.95 & 0.15 & 0.21 & -0.26 & 0.30 \\ 
   \bottomrule
\end{tabularx}



==> Output/Tables/4_Simulation/simtable_240405.tex <==
% latex table generated in R 4.3.1 by xtable 1.8-4 package
% Fri Apr  5 11:53:19 2024
\begin{tabularx}{\linewidth}{L*{15}{Y}}
   \toprule
  \toprule
 & \multicolumn{2}{c}{Sim.-par.} & \multicolumn{5}{c}{Test results} & \multicolumn{4}{c}{$ATET_{Selobs}$} & \multicolumn{4}{c}{$ATET_{DiD}$} \\
 \cmidrule(lr){2-3} \cmidrule(lr){4-8} \cmidrule(lr){9-12} \cmidrule(lr){13-16}
 Learner & $\gamma$ & $\delta$ & $\hat{\theta}$ & Std. & SE & p-val & Reject & Bias & RMSE & SE & E.std  & Bias & RMSE & SE. & E.std \\ \midrule
lasso & 0.000 &    0 & 0.021 & 0.099 & 0.083 & 0.425 & 0.107 & 0.132 & 0.193 & 0.134 & 0.140 & 0.153 & 0.224 & 0.152 & 0.163 \\ 
  randomforest & 0.000 &    0 & -0.023 & 0.109 & 0.095 & 0.452 & 0.090 & 0.694 & 0.706 & 0.135 & 0.128 & 0.672 & 0.685 & 0.140 & 0.134 \\ 
  xgboost & 0.000 &    0 & -0.003 & 0.256 & 0.244 & 0.488 & 0.057 & 0.081 & 0.314 & 0.303 & 0.304 & 0.078 & 0.347 & 0.334 & 0.338 \\ 
  svm & 0.000 &    0 & -0.005 & 0.158 & 0.144 & 0.473 & 0.052 & 0.337 & 0.391 & 0.199 & 0.199 & 0.332 & 0.393 & 0.211 & 0.211 \\ 
  ensemble & 0.000 &    0 & 0.043 & 0.105 & 0.086 & 0.392 & 0.148 & 0.166 & 0.221 & 0.135 & 0.146 & 0.209 & 0.269 & 0.154 & 0.170 \\ 
  parametric & 0.000 &    0 & 0.002 & 0.178 & 0.156 & 0.451 & 0.060 & -0.006 & 0.295 & 0.264 & 0.295 & -0.004 & 0.340 & 0.300 & 0.340 \\ 
  lasso & 0.050 &    0 & -0.026 & 0.098 & 0.083 & 0.442 & 0.112 & 0.179 & 0.226 & 0.134 & 0.138 & 0.153 & 0.222 & 0.151 & 0.160 \\ 
  randomforest & 0.050 &    0 & -0.080 & 0.108 & 0.096 & 0.391 & 0.163 & 0.752 & 0.762 & 0.136 & 0.125 & 0.672 & 0.685 & 0.140 & 0.133 \\ 
  xgboost & 0.050 &    0 & -0.057 & 0.266 & 0.247 & 0.465 & 0.068 & 0.116 & 0.324 & 0.307 & 0.302 & 0.060 & 0.347 & 0.336 & 0.342 \\ 
  svm & 0.050 &    0 & -0.054 & 0.161 & 0.148 & 0.453 & 0.062 & 0.387 & 0.434 & 0.201 & 0.195 & 0.334 & 0.395 & 0.210 & 0.210 \\ 
  ensemble & 0.050 &    0 & -0.002 & 0.102 & 0.087 & 0.447 & 0.106 & 0.211 & 0.256 & 0.135 & 0.144 & 0.209 & 0.266 & 0.154 & 0.165 \\ 
  parametric & 0.050 &    0 & -0.052 & 0.182 & 0.157 & 0.447 & 0.080 & 0.031 & 0.291 & 0.265 & 0.289 & -0.021 & 0.331 & 0.300 & 0.330 \\ 
  lasso & 0.100 &    0 & -0.072 & 0.100 & 0.084 & 0.374 & 0.187 & 0.226 & 0.266 & 0.134 & 0.139 & 0.155 & 0.225 & 0.151 & 0.163 \\ 
  randomforest & 0.100 &    0 & -0.137 & 0.110 & 0.096 & 0.276 & 0.331 & 0.808 & 0.818 & 0.136 & 0.125 & 0.671 & 0.684 & 0.140 & 0.134 \\ 
  xgboost & 0.100 &    0 & -0.101 & 0.271 & 0.254 & 0.451 & 0.079 & 0.181 & 0.347 & 0.303 & 0.297 & 0.080 & 0.343 & 0.333 & 0.334 \\ 
  svm & 0.100 &    0 & -0.100 & 0.161 & 0.150 & 0.414 & 0.113 & 0.438 & 0.479 & 0.199 & 0.193 & 0.338 & 0.398 & 0.207 & 0.211 \\ 
   \bottomrule
\end{tabularx}



==> Output/Tables/4_Simulation/simtable_240425.tex <==
% latex table generated in R 4.3.1 by xtable 1.8-4 package
% Thu Apr 25 16:19:44 2024
\begin{tabularx}{\linewidth}{ccl*{13}{Y}}
   \toprule
  \toprule
 \multicolumn{2}{c}{\textit{Sim.-par.}} &  & \multicolumn{5}{c}{\textit{Test results}} & \multicolumn{4}{c}{\textit{Selobs}} & \multicolumn{4}{c}{\textit{DiD}} \\
 \cmidrule(lr){1-2} \cmidrule(lr){4-8} \cmidrule(lr){9-12} \cmidrule(lr){13-16}
 $\gamma$ & $\delta$ & Learner & $\hat{\theta}$ & Std. & SE & p-val & Reject & Bias & RMSE & SE & E.std  & Bias & RMSE & SE. & E.std \\ 
  \cmidrule(lr){1-2} \cmidrule(lr){3-8} \cmidrule(lr){9-12} \cmidrule(lr){13-16}
 \multirow{6}{*}{0.00} &  \multirow{6}{*}{0.00} & Lasso & 0.021 & 0.099 & 0.083 & 0.425 & 0.107 & 0.132 & 0.193 & 0.134 & 0.140 & 0.153 & 0.224 & 0.152 & 0.163 \\ 
   &  & RF & -0.023 & 0.109 & 0.095 & 0.452 & 0.090 & 0.694 & 0.706 & 0.135 & 0.128 & 0.672 & 0.685 & 0.140 & 0.134 \\ 
   &  & XGBoost & -0.003 & 0.256 & 0.244 & 0.488 & 0.057 & 0.081 & 0.314 & 0.303 & 0.304 & 0.078 & 0.347 & 0.334 & 0.338 \\ 
   &  & SVM & -0.005 & 0.158 & 0.144 & 0.473 & 0.052 & 0.337 & 0.391 & 0.199 & 0.199 & 0.332 & 0.393 & 0.211 & 0.211 \\ 
   &  & Ensemble & 0.043 & 0.105 & 0.086 & 0.392 & 0.148 & 0.166 & 0.221 & 0.135 & 0.146 & 0.209 & 0.269 & 0.154 & 0.170 \\ 
   &  & Parametric & 0.002 & 0.178 & 0.156 & 0.451 & 0.060 & -0.006 & 0.295 & 0.264 & 0.295 & -0.004 & 0.340 & 0.300 & 0.340 \\ 
   \cmidrule(lr){1-2} \cmidrule(lr){3-8} \cmidrule(lr){9-12} \cmidrule(lr){13-16} \multirow{6}{*}{0.05} &  \multirow{6}{*}{0.00} & Lasso & -0.026 & 0.098 & 0.083 & 0.442 & 0.112 & 0.179 & 0.226 & 0.134 & 0.138 & 0.153 & 0.222 & 0.151 & 0.160 \\ 
   &  & RF & -0.080 & 0.108 & 0.096 & 0.391 & 0.163 & 0.752 & 0.762 & 0.136 & 0.125 & 0.672 & 0.685 & 0.140 & 0.133 \\ 
   &  & XGBoost & -0.057 & 0.266 & 0.247 & 0.465 & 0.068 & 0.116 & 0.324 & 0.307 & 0.302 & 0.060 & 0.347 & 0.336 & 0.342 \\ 
   &  & SVM & -0.054 & 0.161 & 0.148 & 0.453 & 0.062 & 0.387 & 0.434 & 0.201 & 0.195 & 0.334 & 0.395 & 0.210 & 0.210 \\ 
   &  & Ensemble & -0.002 & 0.102 & 0.087 & 0.447 & 0.106 & 0.211 & 0.256 & 0.135 & 0.144 & 0.209 & 0.266 & 0.154 & 0.165 \\ 
   &  & Parametric & -0.052 & 0.182 & 0.157 & 0.447 & 0.080 & 0.031 & 0.291 & 0.265 & 0.289 & -0.021 & 0.331 & 0.300 & 0.330 \\ 
   \cmidrule(lr){1-2} \cmidrule(lr){3-8} \cmidrule(lr){9-12} \cmidrule(lr){13-16} \multirow{6}{*}{0.10} &  \multirow{6}{*}{0.00} & Lasso & -0.072 & 0.100 & 0.084 & 0.374 & 0.187 & 0.226 & 0.266 & 0.134 & 0.139 & 0.155 & 0.225 & 0.151 & 0.163 \\ 
   &  & RF & -0.137 & 0.110 & 0.096 & 0.276 & 0.331 & 0.808 & 0.818 & 0.136 & 0.125 & 0.671 & 0.684 & 0.140 & 0.134 \\ 
   &  & XGBoost & -0.101 & 0.271 & 0.254 & 0.451 & 0.079 & 0.181 & 0.347 & 0.303 & 0.297 & 0.080 & 0.343 & 0.333 & 0.334 \\ 
   &  & SVM & -0.100 & 0.161 & 0.150 & 0.414 & 0.113 & 0.438 & 0.479 & 0.199 & 0.193 & 0.338 & 0.398 & 0.207 & 0.211 \\ 
   \bottomrule
\end{tabularx}


==> Output/Tables/4_Simulation/simtable_240429.tex <==
% latex table generated in R 4.3.1 by xtable 1.8-4 package
% Mon Apr 29 16:47:05 2024
\begin{tabularx}{\linewidth}{cccl*{13}{Y}}
   \toprule
  \toprule
 \multicolumn{3}{c}{\textit{Sim.-par.}} & & \multicolumn{5}{c}{\textit{Test results}} & \multicolumn{4}{c}{\textit{Selobs}} & \multicolumn{4}{c}{\textit{DiD}} \\
 \cmidrule(lr){1-3} \cmidrule(lr){5-9} \cmidrule(lr){10-13} \cmidrule(lr){14-17}
 $N$ & $\gamma$ & $\delta$ & Learner & $\hat{\theta}$ & Std. & SE & p-val & Reject & Bias & RMSE & SE & E.std  & Bias & RMSE & SE. & E.std \\ \midrule
 \multirow{6}{*}{1,000} &  \multirow{6}{*}{0.00} &  \multirow{6}{*}{0.00} & Ensemble & 0.043 & 0.105 & 0.086 & 0.392 & 0.148 & 0.166 & 0.221 & 0.135 & 0.146 & 0.209 & 0.269 & 0.154 & 0.170 \\ 
   &  &  & Lasso & 0.021 & 0.099 & 0.083 & 0.425 & 0.107 & 0.132 & 0.193 & 0.134 & 0.140 & 0.153 & 0.224 & 0.152 & 0.163 \\ 
   &  &  & Parametric & 0.002 & 0.178 & 0.156 & 0.451 & 0.060 & -0.006 & 0.295 & 0.264 & 0.295 & -0.004 & 0.340 & 0.300 & 0.340 \\ 
   &  &  & RF & -0.023 & 0.109 & 0.095 & 0.452 & 0.090 & 0.694 & 0.706 & 0.135 & 0.128 & 0.672 & 0.685 & 0.140 & 0.134 \\ 
   &  &  & SVM & -0.005 & 0.158 & 0.144 & 0.473 & 0.052 & 0.337 & 0.391 & 0.199 & 0.199 & 0.332 & 0.393 & 0.211 & 0.211 \\ 
   &  &  & XGBoost & -0.003 & 0.256 & 0.244 & 0.488 & 0.057 & 0.081 & 0.314 & 0.303 & 0.304 & 0.078 & 0.347 & 0.334 & 0.338 \\ 
   \cmidrule(lr){1-3} \cmidrule(lr){4-9} \cmidrule(lr){10-13} \cmidrule(lr){14-17} \multirow{6}{*}{1,000} &  \multirow{6}{*}{0.00} &  \multirow{6}{*}{0.25} & Ensemble & -0.376 & 0.117 & 0.104 & 0.020 & 0.927 & 0.185 & 0.240 & 0.142 & 0.152 & -0.190 & 0.251 & 0.145 & 0.164 \\ 
   &  &  & Lasso & -0.405 & 0.106 & 0.100 & 0.012 & 0.950 & 0.149 & 0.210 & 0.139 & 0.147 & -0.256 & 0.301 & 0.144 & 0.159 \\ 
   &  &  & Parametric & -0.445 & 0.246 & 0.221 & 0.145 & 0.559 & 0.003 & 0.285 & 0.270 & 0.285 & -0.441 & 0.542 & 0.289 & 0.315 \\ 
   &  &  & RF & -0.592 & 0.104 & 0.099 & 0.000 & 1.000 & 0.899 & 0.907 & 0.138 & 0.122 & 0.307 & 0.336 & 0.137 & 0.136 \\ 
   &  &  & SVM & -0.473 & 0.168 & 0.174 & 0.058 & 0.793 & 0.435 & 0.481 & 0.217 & 0.204 & -0.037 & 0.209 & 0.203 & 0.205 \\ 
   &  &  & XGBoost & -0.480 & 0.313 & 0.317 & 0.237 & 0.368 & 0.112 & 0.322 & 0.317 & 0.302 & -0.368 & 0.503 & 0.340 & 0.343 \\ 
   \cmidrule(lr){1-3} \cmidrule(lr){4-9} \cmidrule(lr){10-13} \cmidrule(lr){14-17} \multirow{6}{*}{1,000} &  \multirow{6}{*}{0.25} &  \multirow{6}{*}{0.00} & Ensemble & -0.182 & 0.106 & 0.092 & 0.154 & 0.528 & 0.387 & 0.413 & 0.136 & 0.145 & 0.205 & 0.263 & 0.150 & 0.164 \\ 
   &  &  & Lasso & -0.203 & 0.098 & 0.088 & 0.104 & 0.654 & 0.352 & 0.378 & 0.135 & 0.138 & 0.149 & 0.217 & 0.149 & 0.158 \\ 
   &  &  & Parametric & -0.249 & 0.198 & 0.177 & 0.260 & 0.325 & 0.213 & 0.362 & 0.267 & 0.293 & -0.036 & 0.337 & 0.295 & 0.336 \\ 
   &  &  & RF & -0.307 & 0.108 & 0.097 & 0.033 & 0.877 & 0.966 & 0.974 & 0.137 & 0.122 & 0.659 & 0.672 & 0.139 & 0.134 \\ 
   &  &  & SVM & -0.247 & 0.158 & 0.154 & 0.220 & 0.389 & 0.583 & 0.614 & 0.200 & 0.195 & 0.336 & 0.395 & 0.203 & 0.207 \\ 
   &  &  & XGBoost & -0.251 & 0.279 & 0.272 & 0.370 & 0.179 & 0.310 & 0.427 & 0.305 & 0.294 & 0.060 & 0.348 & 0.335 & 0.342 \\ 
   \bottomrule
\end{tabularx}



==> Output/Tables/4_Simulation/simtable_240513.tex <==
% latex table generated in R 4.3.1 by xtable 1.8-4 package
% Mon May 13 11:04:08 2024
\begin{tabularx}{\linewidth}{cccl*{13}{Y}}
   \toprule
  \toprule
 \multicolumn{3}{c}{\textit{Sim.-par.}} & & \multicolumn{5}{c}{\textit{Test results}} & \multicolumn{4}{c}{\textit{Selobs}} & \multicolumn{4}{c}{\textit{DiD}} \\
 \cmidrule(lr){1-3} \cmidrule(lr){5-9} \cmidrule(lr){10-13} \cmidrule(lr){14-17}
  $\gamma$ & $\delta$ & $N$ & Learner & $\hat{\theta}$ & Std. & SE & p-val & Reject & Bias & RMSE & SE & E.std  & Bias & RMSE & SE. & E.std \\ \midrule
 \multirow{8}{*}{0.00} &  \multirow{8}{*}{0.00} &  \multirow{6}{*}{1,000} & Ensemble & 0.043 & 0.105 & 0.086 & 0.392 & 0.148 & 0.166 & 0.221 & 0.135 & 0.146 & 0.209 & 0.269 & 0.154 & 0.170 \\ 
   &  &  & Lasso & 0.021 & 0.099 & 0.083 & 0.425 & 0.107 & 0.132 & 0.193 & 0.134 & 0.140 & 0.153 & 0.224 & 0.152 & 0.163 \\ 
   &  &  & Parametric & 0.002 & 0.178 & 0.156 & 0.451 & 0.060 & -0.006 & 0.295 & 0.264 & 0.295 & -0.004 & 0.340 & 0.300 & 0.340 \\ 
   &  &  & RF & -0.023 & 0.109 & 0.095 & 0.452 & 0.090 & 0.694 & 0.706 & 0.135 & 0.128 & 0.672 & 0.685 & 0.140 & 0.134 \\ 
   &  &  & SVM & -0.005 & 0.158 & 0.144 & 0.473 & 0.052 & 0.337 & 0.391 & 0.199 & 0.199 & 0.332 & 0.393 & 0.211 & 0.211 \\ 
   &  &  & XGBoost & -0.003 & 0.256 & 0.244 & 0.488 & 0.057 & 0.081 & 0.314 & 0.303 & 0.304 & 0.078 & 0.347 & 0.334 & 0.338 \\ 
   \cmidrule(lr){3-3} \cmidrule(lr){4-9} \cmidrule(lr){10-13} \cmidrule(lr){14-17} &  &  \multirow{2}{*}{4,000} & Lasso & 0.007 & 0.044 & 0.040 & 0.480 & 0.075 & 0.032 & 0.078 & 0.069 & 0.071 & 0.038 & 0.091 & 0.079 & 0.083 \\ 
   &  &  & Parametric & -0.001 & 0.052 & 0.050 & 0.486 & 0.064 & -0.005 & 0.090 & 0.087 & 0.090 & -0.006 & 0.105 & 0.100 & 0.104 \\ 
   \cmidrule(lr){1-3} \cmidrule(lr){4-9} \cmidrule(lr){10-13} \cmidrule(lr){14-17} \multirow{8}{*}{0.00} &  \multirow{8}{*}{0.25} &  \multirow{6}{*}{1,000} & Ensemble & -0.376 & 0.117 & 0.104 & 0.020 & 0.927 & 0.185 & 0.240 & 0.142 & 0.152 & -0.190 & 0.251 & 0.145 & 0.164 \\ 
   &  &  & Lasso & -0.405 & 0.106 & 0.100 & 0.012 & 0.950 & 0.149 & 0.210 & 0.139 & 0.147 & -0.256 & 0.301 & 0.144 & 0.159 \\ 
   &  &  & Parametric & -0.445 & 0.246 & 0.221 & 0.145 & 0.559 & 0.003 & 0.285 & 0.270 & 0.285 & -0.441 & 0.542 & 0.289 & 0.315 \\ 
   &  &  & RF & -0.592 & 0.104 & 0.099 & 0.000 & 1.000 & 0.899 & 0.907 & 0.138 & 0.122 & 0.307 & 0.336 & 0.137 & 0.136 \\ 
   &  &  & SVM & -0.473 & 0.168 & 0.174 & 0.058 & 0.793 & 0.435 & 0.481 & 0.217 & 0.204 & -0.037 & 0.209 & 0.203 & 0.205 \\ 
   &  &  & XGBoost & -0.480 & 0.313 & 0.317 & 0.237 & 0.368 & 0.112 & 0.322 & 0.317 & 0.302 & -0.368 & 0.503 & 0.340 & 0.343 \\ 
   \cmidrule(lr){3-3} \cmidrule(lr){4-9} \cmidrule(lr){10-13} \cmidrule(lr){14-17} &  &  \multirow{2}{*}{4,000} & Lasso & -0.408 & 0.052 & 0.051 & 0.000 & 1.000 & 0.038 & 0.083 & 0.072 & 0.074 & -0.370 & 0.379 & 0.075 & 0.081 \\ 
   &  &  & Parametric & -0.409 & 0.066 & 0.063 & 0.000 & 1.000 & -0.001 & 0.091 & 0.089 & 0.091 & -0.410 & 0.422 & 0.092 & 0.097 \\ 
   \cmidrule(lr){1-3} \cmidrule(lr){4-9} \cmidrule(lr){10-13} \cmidrule(lr){14-17} \multirow{8}{*}{0.25} &  \multirow{8}{*}{0.00} &  \multirow{6}{*}{1,000} & Ensemble & -0.182 & 0.106 & 0.092 & 0.154 & 0.528 & 0.387 & 0.413 & 0.136 & 0.145 & 0.205 & 0.263 & 0.150 & 0.164 \\ 
   &  &  & Lasso & -0.203 & 0.098 & 0.088 & 0.104 & 0.654 & 0.352 & 0.378 & 0.135 & 0.138 & 0.149 & 0.217 & 0.149 & 0.158 \\ 
   &  &  & Parametric & -0.249 & 0.198 & 0.177 & 0.260 & 0.325 & 0.213 & 0.362 & 0.267 & 0.293 & -0.036 & 0.337 & 0.295 & 0.336 \\ 
   &  &  & RF & -0.307 & 0.108 & 0.097 & 0.033 & 0.877 & 0.966 & 0.974 & 0.137 & 0.122 & 0.659 & 0.672 & 0.139 & 0.134 \\ 
   &  &  & SVM & -0.247 & 0.158 & 0.154 & 0.220 & 0.389 & 0.583 & 0.614 & 0.200 & 0.195 & 0.336 & 0.395 & 0.203 & 0.207 \\ 
   &  &  & XGBoost & -0.251 & 0.279 & 0.272 & 0.370 & 0.179 & 0.310 & 0.427 & 0.305 & 0.294 & 0.060 & 0.348 & 0.335 & 0.342 \\ 
   \cmidrule(lr){3-3} \cmidrule(lr){4-9} \cmidrule(lr){10-13} \cmidrule(lr){14-17} &  &  \multirow{2}{*}{4,000} & Lasso & -0.213 & 0.045 & 0.043 & 0.001 & 0.992 & 0.253 & 0.262 & 0.069 & 0.069 & 0.040 & 0.089 & 0.077 & 0.079 \\ 
   &  &  & Parametric & -0.220 & 0.056 & 0.053 & 0.005 & 0.975 & 0.218 & 0.235 & 0.086 & 0.087 & -0.002 & 0.099 & 0.096 & 0.099 \\ 
   \bottomrule
\end{tabularx}



==> Output/Tables/4_Simulation/simtable_240524_old.tex <==
% latex table generated in R 4.3.1 by xtable 1.8-4 package
% Fri May 24 11:29:33 2024
\begin{tabularx}{\linewidth}{cccl*{13}{Y}}
   \toprule
  \toprule
 \multicolumn{3}{c}{\textit{Sim.-par.}} & & \multicolumn{5}{c}{\textit{Test results}} & \multicolumn{4}{c}{\textit{Unconf}} & \multicolumn{4}{c}{\textit{DiD}} \\
 \cmidrule(lr){1-3} \cmidrule(lr){5-9} \cmidrule(lr){10-13} \cmidrule(lr){14-17}
  $\gamma$ & $\delta$ & $n$ & Learner & $\hat{\theta}$ & Std. & SE & p-val & Reject & Bias & RMSE & SE & E.std  & Bias & RMSE & SE. & E.std \\ \midrule
 \multirow{10}{*}{0.00} &  \multirow{10}{*}{0.00} &  \multirow{5}{*}{1,000} & Ensemble & 0.043 & 0.105 & 0.086 & 0.392 & 0.148 & 0.166 & 0.221 & 0.135 & 0.146 & 0.209 & 0.269 & 0.154 & 0.170 \\ 
   &  &  & Lasso & 0.021 & 0.099 & 0.083 & 0.425 & 0.107 & 0.132 & 0.193 & 0.134 & 0.140 & 0.153 & 0.224 & 0.152 & 0.163 \\ 
   &  &  & Parametric & 0.002 & 0.178 & 0.156 & 0.451 & 0.060 & -0.006 & 0.295 & 0.264 & 0.295 & -0.004 & 0.340 & 0.300 & 0.340 \\ 
   &  &  & RF & -0.023 & 0.109 & 0.095 & 0.452 & 0.090 & 0.694 & 0.706 & 0.135 & 0.128 & 0.672 & 0.685 & 0.140 & 0.134 \\ 
   &  &  & SVM & -0.005 & 0.158 & 0.144 & 0.473 & 0.052 & 0.337 & 0.391 & 0.199 & 0.199 & 0.332 & 0.393 & 0.211 & 0.211 \\ 
   \cmidrule(lr){3-3} \cmidrule(lr){4-9} \cmidrule(lr){10-13} \cmidrule(lr){14-17} &  &  \multirow{5}{*}{4,000} & Ensemble & 0.020 & 0.052 & 0.039 & 0.390 & 0.157 & 0.044 & 0.089 & 0.067 & 0.078 & 0.064 & 0.112 & 0.076 & 0.091 \\ 
   &  &  & Lasso & 0.007 & 0.044 & 0.040 & 0.480 & 0.075 & 0.032 & 0.078 & 0.069 & 0.071 & 0.038 & 0.091 & 0.079 & 0.083 \\ 
   &  &  & Parametric & -0.001 & 0.052 & 0.050 & 0.486 & 0.064 & -0.005 & 0.090 & 0.087 & 0.090 & -0.006 & 0.105 & 0.100 & 0.104 \\ 
   &  &  & RF & -0.021 & 0.052 & 0.046 & 0.434 & 0.120 & 0.533 & 0.537 & 0.067 & 0.063 & 0.511 & 0.516 & 0.070 & 0.068 \\ 
   &  &  & SVM & 0.004 & 0.063 & 0.060 & 0.488 & 0.061 & 0.151 & 0.175 & 0.088 & 0.089 & 0.155 & 0.184 & 0.098 & 0.099 \\ 
   \cmidrule(lr){1-3} \cmidrule(lr){4-9} \cmidrule(lr){10-13} \cmidrule(lr){14-17} \multirow{10}{*}{0.25} &  \multirow{10}{*}{0.00} &  \multirow{5}{*}{1,000} & Ensemble & -0.182 & 0.106 & 0.092 & 0.154 & 0.528 & 0.387 & 0.413 & 0.136 & 0.145 & 0.205 & 0.263 & 0.150 & 0.164 \\ 
   &  &  & Lasso & -0.203 & 0.098 & 0.088 & 0.104 & 0.654 & 0.352 & 0.378 & 0.135 & 0.138 & 0.149 & 0.217 & 0.149 & 0.158 \\ 
   &  &  & Parametric & -0.249 & 0.198 & 0.177 & 0.260 & 0.325 & 0.213 & 0.362 & 0.267 & 0.293 & -0.036 & 0.337 & 0.295 & 0.336 \\ 
   &  &  & RF & -0.307 & 0.108 & 0.097 & 0.033 & 0.877 & 0.966 & 0.974 & 0.137 & 0.122 & 0.659 & 0.672 & 0.139 & 0.134 \\ 
   &  &  & SVM & -0.247 & 0.158 & 0.154 & 0.220 & 0.389 & 0.583 & 0.614 & 0.200 & 0.195 & 0.336 & 0.395 & 0.203 & 0.207 \\ 
   \cmidrule(lr){3-3} \cmidrule(lr){4-9} \cmidrule(lr){10-13} \cmidrule(lr){14-17} &  &  \multirow{5}{*}{4,000} & Ensemble & -0.196 & 0.051 & 0.042 & 0.003 & 0.986 & 0.262 & 0.273 & 0.067 & 0.078 & 0.066 & 0.111 & 0.075 & 0.089 \\ 
   &  &  & Lasso & -0.213 & 0.045 & 0.043 & 0.001 & 0.992 & 0.253 & 0.262 & 0.069 & 0.069 & 0.040 & 0.089 & 0.077 & 0.079 \\ 
   &  &  & Parametric & -0.220 & 0.056 & 0.053 & 0.005 & 0.975 & 0.218 & 0.235 & 0.086 & 0.087 & -0.002 & 0.099 & 0.096 & 0.099 \\ 
   &  &  & RF & -0.304 & 0.053 & 0.047 & 0.000 & 1.000 & 0.803 & 0.805 & 0.068 & 0.062 & 0.499 & 0.503 & 0.069 & 0.066 \\ 
   &  &  & SVM & -0.228 & 0.064 & 0.065 & 0.017 & 0.926 & 0.384 & 0.394 & 0.088 & 0.087 & 0.156 & 0.182 & 0.094 & 0.095 \\ 
   \cmidrule(lr){1-3} \cmidrule(lr){4-9} \cmidrule(lr){10-13} \cmidrule(lr){14-17} \multirow{9}{*}{0.00} &  \multirow{9}{*}{0.25} &  \multirow{5}{*}{1,000} & Ensemble & -0.376 & 0.117 & 0.104 & 0.020 & 0.927 & 0.185 & 0.240 & 0.142 & 0.152 & -0.190 & 0.251 & 0.145 & 0.164 \\ 
   &  &  & Lasso & -0.405 & 0.106 & 0.100 & 0.012 & 0.950 & 0.149 & 0.210 & 0.139 & 0.147 & -0.256 & 0.301 & 0.144 & 0.159 \\ 
   &  &  & Parametric & -0.445 & 0.246 & 0.221 & 0.145 & 0.559 & 0.003 & 0.285 & 0.270 & 0.285 & -0.441 & 0.542 & 0.289 & 0.315 \\ 
   &  &  & RF & -0.592 & 0.104 & 0.099 & 0.000 & 1.000 & 0.899 & 0.907 & 0.138 & 0.122 & 0.307 & 0.336 & 0.137 & 0.136 \\ 
   \cmidrule(lr){3-3} \cmidrule(lr){4-9} \cmidrule(lr){10-13} \cmidrule(lr){14-17} &  &  & SVM & -0.473 & 0.168 & 0.174 & 0.058 & 0.793 & 0.435 & 0.481 & 0.217 & 0.204 & -0.037 & 0.209 & 0.203 & 0.205 \\ 
   &  &  \multirow{4}{*}{4,000} & Lasso & -0.408 & 0.052 & 0.051 & 0.000 & 1.000 & 0.038 & 0.083 & 0.072 & 0.074 & -0.370 & 0.379 & 0.075 & 0.081 \\ 
   &  &  & Parametric & -0.409 & 0.066 & 0.063 & 0.000 & 1.000 & -0.001 & 0.091 & 0.089 & 0.091 & -0.410 & 0.422 & 0.092 & 0.097 \\ 
   &  &  & RF & -0.574 & 0.054 & 0.049 & 0.000 & 1.000 & 0.708 & 0.711 & 0.068 & 0.064 & 0.134 & 0.151 & 0.068 & 0.069 \\ 
   &  &  & SVM & -0.433 & 0.072 & 0.075 & 0.001 & 0.995 & 0.195 & 0.217 & 0.096 & 0.093 & -0.237 & 0.256 & 0.091 & 0.095 \\ 
   \bottomrule
\end{tabularx}


